MiniGPT-3D: Efficiently Aligning 3D Point Clouds with Large Language Models using 2D Priors

Large 2D vision-language models (2D-LLMs) have gained significant attention by bridging Large Language Models (LLMs) with images using a simple projector. Inspired by their success, large 3D point cloud-language models (3D-LLMs) also integrate point clouds into LLMs. However, directly aligning point clouds with LLM requires expensive training costs, typically in hundreds of GPU-hours on A100, which hinders the development of 3D-LLMs. In this paper, we introduce MiniGPT-3D, an efficient and powerful 3D-LLM that achieves multiple SOTA results while training for only 27 hours on one RTX 3090. Specifically, we propose to align 3D point clouds with LLMs using 2D priors from 2D-LLMs, which can leverage the similarity between 2D and 3D visual information. We introduce a novel four-stage training strategy for modality alignment in a cascaded way, and a mixture of query experts module to adaptively aggregate features with high efficiency. Moreover, we utilize parameter-efficient fine-tuning methods LoRA and Norm fine-tuning, resulting in only 47.8M learnable parameters, which is up to 260x fewer than existing methods. Extensive experiments show that MiniGPT-3D achieves SOTA on 3D object classification and captioning tasks, with significantly cheaper training costs. Notably, MiniGPT-3D gains an 8.12 increase on GPT-4 evaluation score for the challenging object captioning task compared to ShapeLLM-13B, while the latter costs 160 total GPU-hours on 8 A800. We are the first to explore the efficient 3D-LLM, offering new insights to the community. Code and weights are available at https://github.com/TangYuan96/MiniGPT-3D.

==> samples/sup_material/Tab/params.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[]

  \caption{Parameters and trainable attributes of each module in  MiniGPT-3D.}

\begin{NiceTabular}{lrcr}
\toprule
\textbf{\begin{tabular}[c]{@{}l@{}}Trainable\\ Module\end{tabular}}  & \textbf{Params}   & \textbf{\begin{tabular}[c]{@{}c@{}}Frozen\\ Module\end{tabular}}  & \textbf{Params}   \\ \midrule
\rowcolor[HTML]{EFEFEF} 
\begin{tabular}[c]{@{}l@{}}Point Cloud Projection \\ Layer (MLP)\end{tabular} &  {\color[HTML]{ff8954} 1.4 M}  & \begin{tabular}[c]{@{}c@{}}PC \\  Encoder\end{tabular}  & {\color[HTML]{02b7db} 21.9 M}  \\
\begin{tabular}[c]{@{}l@{}}Norm \& LoRA\\ of Q-Former\end{tabular}  &  {\color[HTML]{ff8954} 0.7 M}  & Q-Former  & {\color[HTML]{02b7db} 105 M } \\
\rowcolor[HTML]{EFEFEF} 
Modality Projector  &  {\color[HTML]{ff8954} 13.7 M}  & LLM (Phi-2)  &{\color[HTML]{02b7db}  2780 M}  \\ 
Mixture of Query Experts  &  {\color[HTML]{ff8954} 0.4 M}  & - & - \\ 
\rowcolor[HTML]{EFEFEF} 
Norm \& LoRA  of LLM  &  {\color[HTML]{ff8954} 31.6 M}  & -   & -  \\ \midrule
\textbf{Total   Parameters }  & {\color[HTML]{ff8954} \textbf{47.8 M}} & -   & {\color[HTML]{02b7db} \textbf{2907 M}}  \\ \bottomrule
\end{NiceTabular}
\label{sup_tab:total_para}
\end{table}

==> samples/tables/1_abl_train_progress.tex <==



\begin{table}[t]
    \centering
    % \setlength\tabcolsep{6pt}
    % \setlength{\abovecaptionskip}{0.2cm}  
    % \setlength{\belowcaptionskip}{-0.4cm}
    % \renewcommand{\arraystretch}{1.05}
    
\caption{Ablation on four-stage training process.
   }
    \resizebox*{0.8\linewidth}{!}{
\begin{tabular}{c|ccccc}
\hline
Row No. & Stage  I & Stage II & Stage III & Stage IV & Acc. \\ \hline
 1  & $\surd$ &                      &                      &                      & 39.10                     \\
 2  & $\surd$ & $\surd$ &                      &                      & 55.92                     \\
 3  & $\surd$ & $\surd$ &   $\surd$                   &                      & 59.10                     \\
\rowcolor[HTML]{EFEFEF} 
 4  & $\surd$ & $\surd$ & $\surd$ & $\surd$ & \textbf{60.56}                     \\
 5  & $\surd$ &          & $\surd$ & $\surd$ & 52.81                     \\
6  &          & $\surd$ & $\surd$ & $\surd$ & 58.46                     \\
7   & $\surd$ & $\surd$ &         & $\surd$ &                       \\
 \hline
\end{tabular}
}
   \label{tb:ablation_train_progress}
\end{table}



 
% \begin{table}[t]
%     \centering
%     \setlength\tabcolsep{10pt}
%     % \setlength{\abovecaptionskip}{0.2cm}  
%     % \setlength{\belowcaptionskip}{-0.4cm}
%     \renewcommand{\arraystretch}{1.05}
    

%     \resizebox*{\linewidth}{!}{
% \begin{tabular}{c|ccccc}
% \hline
% Row No. & Stage  I & Stage II & Stage III & Stage IV & Acc. \\ \hline
%  1  & $\surd$ &                      &                      &                      & 39.10                     \\
%  2  & $\surd$ & $\surd$ &                      &                      & 55.92                     \\
%  3  & $\surd$ & $\surd$ &   $\surd$                   &                      & 59.10                     \\
% \rowcolor[HTML]{EFEFEF} 
%  4  & $\surd$ & $\surd$ & $\surd$ & $\surd$ & \textbf{60.56}                     \\
%  5  & $\surd$ &                      & $\surd$ & $\surd$ & 52.81                     \\
%  6  & $\surd$ &                      & $\surd$ &                      & 52.62                     \\
% 7   &                      & $\surd$ & $\surd$ & $\surd$ & 58.46                     \\
% 8   &                      & $\surd$ & $\surd$ &                      & 58.05                     \\
%  9  &                      & $\surd$ &                      & $\surd$ & 48.88                     \\
%  10  &                      & $\surd$ &                      &                      & 56.67                     \\ \hline
% \end{tabular}
% }
% \caption{Ablation on four-stage training process.
%    }
%    \label{tb:ablation_train_progress}
% \end{table}

==> samples/tables/2_abl_tinygpt_v_weight.tex <==
  
\begin{table}[t]
\caption{Ablation on pre-trained weight from 2D-LLM.
   }
  \resizebox*{0.48\linewidth}{!}{
\begin{tabular}{lc}
\hline
\begin{tabular}[c]{@{}l@{}}Pre-trained Weights \\ from 2D-LLM\end{tabular}                           & Acc.      \\ \hline
\rowcolor[HTML]{EFEFEF} 
Use All (Stage II - IV)                                                                              & \textbf{58.46} \\
- Norm and LoRA for LLM                                                                             &                \\
\rowcolor[HTML]{EFEFEF} 
- Modality Projector                                                                                 &                \\
\begin{tabular}[c]{@{}l@{}}- Norm and LoRA for LLM\\ - Modality Projector\end{tabular}              & 49.04          \\
\rowcolor[HTML]{EFEFEF} 
\begin{tabular}[c]{@{}l@{}}- Norm and LoRA for LLM\\ - Modality Projector\\ - Q-Former\end{tabular} & OOM            \\ \hline
\end{tabular}
}
   \label{tab: ablation_train_progress}
\end{table}

==> samples/tables/3_abl_finetuned_moduls_qformer.tex <==
\begin{table}[t]
     \centering
    % \setlength\tabcolsep{2pt}
    % \setlength{\abovecaptionskip}{0.2cm}  
    % \setlength{\belowcaptionskip}{-0.4cm}
    % \renewcommand{\arraystretch}{0.95}
    

\caption{Ablation on fine-tuned modules in Q-Former.
   }
    \resizebox*{0.48\linewidth}{!}{
\begin{tabular}{cccc}
\hline
\multicolumn{2}{c}{LoRA} & \multirow{2}{*}{Norm} & \multirow{2}{*}{Acc.} \\ \cline{1-2}
Q, K, V       & Dense      &                       &                           \\ \hline
                &         &                          & 58.18                      \\
 $\surd$              &         &                          & 59.85                      \\
 $\surd$              & $\surd$       &                          & 59.97                      \\
\rowcolor[HTML]{EFEFEF} 
 $\surd$              &         & $\surd$                        & \textbf{60.56}                     \\
 $\surd$              & $\surd$       & $\surd$                        & 60.14                      \\ \hline
\end{tabular}
}
   \label{tab:abl_fine-tuned_modules_of_Q-Former}
\end{table}

==> samples/tables/4_abl_stage_query_expert.tex <==
\begin{table}[t]

    \centering
    % \setlength\tabcolsep{3pt}
    % % \setlength{\abovecaptionskip}{0.2cm}  
    % % \setlength{\belowcaptionskip}{-0.4cm}
    % \renewcommand{\arraystretch}{1.05}
    

\caption{Ablation on training stages using MQE.}
 \resizebox*{0.65\linewidth}{!}{
\begin{tabular}{ccccc}
\hline
Stage I & Stage II & Stage III & Stage IV & Acc. \\ \hline
 $\surd$             & $\surd$             & $\surd$            & $\surd$            & 58.83                      \\
              & $\surd$             & $\surd$            & $\surd$            & 60.25                      \\
               &               & $\surd$            & $\surd$            & 59.50                      \\
\rowcolor[HTML]{EFEFEF} 
               &               &              & $\surd$            & \textbf{60.56}             \\ \hline
\end{tabular}
}
   \label{tb:ablation_train_stages_query_expert}
 
\end{table}

==> samples/tables/5_abl_router_type.tex <==

\begin{table}[t]
    \centering
    % \setlength\tabcolsep{6pt}
    % \setlength{\abovecaptionskip}{0.2cm}  
    % \setlength{\belowcaptionskip}{-0.4cm}
    % \renewcommand{\arraystretch}{0.95}
    
\caption{Ablation on router type.
   }
    \resizebox*{0.35\linewidth}{!}{
\begin{tabular}{cc}
\hline
Type     & Acc.       \\ \hline
Constant Router & 60.10          \\
\rowcolor[HTML]{EFEFEF} 
Sparse Router   & \textbf{60.56} \\
Soft Router     & 60.31          \\ \hline
\end{tabular}
}
   \label{tab: ablation_routet_type}
\end{table}


==> samples/tables/7_abl_num_query_expert.tex <==

\begin{table}[t]
    \centering
    % \setlength\tabcolsep{6pt}
    % \setlength{\abovecaptionskip}{0.2cm}  
    % \setlength{\belowcaptionskip}{-0.4cm}
    % \renewcommand{\arraystretch}{0.95}
    
\caption{Ablation on the number of query experts.
   }
    \resizebox*{0.23\linewidth}{!}{
\begin{tabular}{cc}
\hline
Num. & Acc.       \\ \hline
1    & 59.19          \\
3    & 59.66          \\
6    & 59.14          \\
\rowcolor[HTML]{EFEFEF} 
8    & \textbf{60.56} \\
10   & 59.85          \\ \hline
\end{tabular}
}
   \label{tab: ablation_num_query_expert}
\end{table}

==> samples/tables/8_abl_pc_linear.tex <==
\begin{table}[t]
    \centering
    % \setlength\tabcolsep{4pt}
    % \setlength{\abovecaptionskip}{0.2cm}  
    % \setlength{\belowcaptionskip}{-0.4cm}
    % \renewcommand{\arraystretch}{0.95}
    
\caption{Ablation on number of  the point cloud projection layers.
   }
    \resizebox*{0.26\linewidth}{!}{
\begin{tabular}{cc}
\hline
\begin{tabular}[c]{@{}c@{}}Number \\of layers\end{tabular} & Acc. \\ \hline
1                & 57.02          \\
\rowcolor[HTML]{EFEFEF} 
2                & \textbf{60.56} \\
3                & 59.20          \\ \hline
\end{tabular}
}

   \label{tab: ablation_pc_linear}
\end{table}



==> samples/tables/ab_all_2_n.tex <==
\begin{table*}[t] 
    \begin{minipage}[b]{0.24\linewidth}  
     \centering
 
        \resizebox*{\linewidth}{!}{
            \begin{tabular}{cccc}
            \hline
            \multicolumn{2}{c}{LoRA} & \multirow{2}{*}{Norm} & \multirow{2}{*}{Acc.} \\ \cline{1-2}
            Q, K, V       & Dense      &                       &                           \\ \hline
                            &         &                          & 58.18                      \\
             $\surd$              &         &                          & 59.85                      \\
             $\surd$              & $\surd$       &                          & 59.97                      \\
            \rowcolor[HTML]{EFEFEF} 
             $\surd$              &         & $\surd$                        & \textbf{60.56}                     \\
             $\surd$              & $\surd$       & $\surd$                        & 60.14                      \\ \hline
            \end{tabular}
            }
            
            \caption{Ablation on fine-tuned modules in Q-Former.
               }
               \label{tab:abl_fine-tuned_modules_of_Q-Former}
        
  \end{minipage}%  
     \hfill % 使用\hfill来填充剩余的水平空间  
  %  
  \begin{minipage}[b]{0.2\linewidth}  
    \centering

    \resizebox*{0.57\linewidth}{!}{
        \begin{tabular}{cc}
        \hline
        Num. & Acc.       \\ \hline
        1    & 59.19          \\
        3    & 59.66          \\
        6    & 59.14          \\
        \rowcolor[HTML]{EFEFEF} 
        8    & \textbf{60.56} \\
        10   & 59.85          \\ \hline
        \end{tabular}
        }
        \caption{Ablation on the number of query experts.
           }
           \label{tab: ablation_num_query_expert}
  \end{minipage}  
        \hfill % 使用\hfill来填充剩余的水平空间  
  %  
  \begin{minipage}[b]{0.3\linewidth}  
    \centering
    \resizebox*{0.6\linewidth}{!}{
        \begin{tabular}{cc}
        \hline
        % \begin{tabular}[c]{@{}c@{}}Number \\of layers\end{tabular} & Acc. \\ \hline
        Number  of layers  & Acc. \\\hline
        1                & 57.02          \\
        \rowcolor[HTML]{EFEFEF} 
        2                & \textbf{60.56} \\
        3                & 59.20          \\ \hline
        \end{tabular}
        }
        \caption{Ablation on the  point  \\ cloud projection layers.
           }
           \label{tab: ablation_pc_linear}
  \end{minipage}
  %
    \hfill % 使用\hfill来填充剩余的水平空间  
  %  
  \begin{minipage}[b]{0.175\linewidth}  
    \centering

    \resizebox*{\linewidth}{!}{
    \begin{tabular}{cc}
    \hline
    Type     & Acc.       \\ \hline
    Constant Router & 60.10          \\
    \rowcolor[HTML]{EFEFEF} 
    Sparse Router   & \textbf{60.56} \\
    Soft Router     & 60.31          \\ \hline
    \end{tabular}
    }
    \caption{Ablation  \\ on router type.
       }
       \label{tab: ablation_routet_type}
  \end{minipage}  
\vspace*{-6mm}
\end{table*}
